AXAI-CDSS : An Affective Explainable AI-Driven Clinical Decision Support System for Cannabis Use

As cannabis use has increased in recent years, researchers have come to rely on sophisticated machine learning models to predict cannabis use behavior and its impact on health. However, many artificial intelligence (AI) models lack transparency and interpretability due to their opaque nature, limiting their trust and adoption in real-world medical applications, such as clinical decision support systems (CDSS). To address this issue, this paper enhances algorithm explainability underlying CDSS by integrating multiple Explainable Artificial Intelligence (XAI) methods and applying causal inference techniques to clarify the model' predictive decisions under various scenarios. By providing deeper interpretability of the XAI outputs using Large Language Models (LLMs), we provide users with more personalized and accessible insights to overcome the challenges posed by AI's "black box" nature. Our system dynamically adjusts feedback based on user queries and emotional states, combining text-based sentiment analysis with real-time facial emotion recognition to ensure responses are empathetic, context-adaptive, and user-centered. This approach bridges the gap between the learning demands of interpretability and the need for intuitive understanding, enabling non-technical users such as clinicians and clinical researchers to interact effectively with AI models.} Ultimately, this approach improves usability, enhances perceived trustworthiness, and increases the impact of CDSS in healthcare applications.

==> section/Research_and_analysis.tex <==
\section{User Feedback}

In addition to the quantitative analysis, participants (i.e., users of the system) provided qualitative feedback, offering insights from their experience in their area of expertise, and made suggestions for improving the system. Overall, many participants cited the system's comprehensive analysis as a major strength. As one participant noted, "The answer is more comprehensive rather than simple data analysis. [P1]" Another participant echoed this sentiment, emphasizing the usefulness of the system in predicting trends based on recent data, stating, "The system provides a detailed analysis of the patient's recent condition, which plays a crucial role in predicting future trends. [P3]"

% \notegb{each quotation needs a PID (e.g. [P2]) at the end of the quoted sentences}"

However, there were also areas where participants felt the system could be improved, particularly in dealing with emergencies and extreme data. One common theme was the desire for a more streamlined and simplified user experience. For example, one user commented, "Response is too wordy. [P4]" Additionally, participants suggested improving the clarity of certain features, with one noting, "I still couldn't understand some features like the SHAP of kurt hr with the explanations. Maybe a clear explanation will helps a lot. [P1]" This reflects the fact that we still need more accessible and user-friendly explanations of complex concepts such as SHAP values and causality.

In terms of the system's ability to provide valuable insights for patients, many participants found the causal learning graphs particularly useful. One user noted, "This is a great start, with potentially helpful information that the clinician and patient would be interested in discussed. The causal inference diagram is especially interesting and intuitive, especially in thinking about how features might be related to intoxication. Great work!  [P8]" This suggests that the system needs to provide a clearer, more concise summary of the patient's condition to enhance real-time decision-making.

\textcolor{black}{Many system users also highlighted areas for improvement in the usability of the system. Some suggested adding interactive features such as the ability to resize images, and adding system usage instructions to enhance the attractiveness of the system to make the system more engaging.} As one participant stated, "Adding some interactive features can improve the user experience. [P3]" Another participant suggested designing a cleaner interface and providing more guidance for new users: "It is recommended to design the system interface to be more concise and add a user guide page. Also, there could be some explanatory features between different function pages to help users understand. [P5]" This reflects a desire for the system to be more intuitive and easier to navigate, especially for those who may not be familiar with the technical aspects of the data. These comments suggest that while the system shows great promise, there are still areas that need further refinement.
